Designing High-Occupancy Toll Lanes: A Game-Theoretic Analysis

In this article, we study the optimal design of High Occupancy Toll (HOT) lanes. The traffic authority determines the road capacity allocation between HOT lanes and ordinary lanes, as well as the toll price charged for travelers using HOT lanes who do not meet the high-occupancy eligibility criteria. We develop a game-theoretic model to analyze the decisions of travelers with heterogeneous preference parameters in values of time and carpool disutilities. These travelers choose between paying or forming carpools to use the HOT lanes, or taking the ordinary lanes. Travelers' welfare depends on the congestion cost of the lane they use, the toll payment, and the carpool disutilities. For highways with a single entrance and exit node, we provide a complete characterization of equilibrium strategies and a comparative statics analysis of how the equilibrium vehicle flow and travel time change with HOT capacity and toll price. We then extend the single segment model to highways with multiple entrance and exit nodes. We extend the equilibrium concept and propose various design objectives considering traffic congestion, toll revenue, and social welfare. Using the data collected from the HOT lane of the California Interstate Highway 880 (I-880), we formulate a convex program to estimate the travel demand and approximate the distribution of travelers' preference parameters. We then compute the optimal toll design of five segments for I-880 for achieve each one of the four objectives, and compare the optimal solution with the current toll pricing.

==> design.tex <==
In this section, we want to find the optimal toll price $\toll$ and the HOT capacity $\rho$ with respect to $4$ different objectives:
minimize total congestion time $\Ltravel(\tau, \rho)$, minimize the total emission $\Lemission(\tau, \rho)$, and maximize total revenue $R(\tau, \rho)$, respectively. The three objectives are defined as follows:
\begin{enumerate}
    \item Average travel time (per agent)
    \[\Ltravel(\toll, \rho) = \strategydiseq[\actiono] \cdot \costo(\flowoeq, 1 - \rho) + (\strategydiseq[\actiont] +\strategydiseq[\actionp])\cdot  \costh(\flowh, \rho)\]
    \item Average emission (per agent)
    \[\Lemission(\toll, \rho) = \strategydiseq[\actiono] \cdot \costo(\flowoeq, 1 - \rho) + (\strategydiseq[\actiont] + \strategydiseq[\actionp]/M)\cdot  \costh(\flowheq, \rho)\]
    \item Average utility cost (per agent)
    \[\Lutility (\toll, \rho) = \iint  C_{s^*(\vot,\disu)}(\strategydiseq;\vot,\disu) \ d\vot d\disu\]
    \item Total Revenue
    \[\Lrevenue(\toll, \rho) = \sigma^*_{\toll} D \cdot \toll \]
\end{enumerate}
where $\strategydiseq$ and $\floweq$ are the equilibrium strategy distribution and equilibrium flow under toll price $\toll$ and HOT capacity $\rho$.

The HOT capacity $\rho$ specifies the fraction of lanes on the highway that are assigned to be HOT lanes, which can only take discrete values. For instance, given a highway of 4 lanes, the number of HOT lanes can be $1$, $2$, or $3$, so $\rho \in \{\frac{1}{4}, \frac{2}{4}, \frac{3}{4}\}$. Since most highways have up to 5 lanes, the value of $\rho$ cannot have too many options. However, the toll price $\tau$ can be any non-negative real number. As a result, we focus on studying the optimal toll price for these three objectives given a fixed HOT capacity. Then, we can repeat the same process for all possible HOT capacities and pick the optimal toll price and the HOT capacity.

We start by uncovering intuitive insights from the analysis of the optimal toll design for linear latency function and simple preference distributions in section \ref{sec:design-simple}. Then we characterize the optimal condition for toll prices under general latency functions and preference distributions in section \ref{sec:design-general}.

\subsection{Linear Latency Functions and Simple Preference Distributions} \label{sec:design-simple}
In this section, we solve for the optimal toll price $\tau$ under three different distributions of the population:
\begin{enumerate}
    \item Homogeneous value of time $\beta$ and Homogeneous carpool disutility $\gamma$,
    \item Homogeneous value of time $\beta$ and uniform carpool disutility $\gamma \sim Unif[\lgamma, \ugamma]$,
    \item Uniform value of time $\beta \sim Unif[\lbeta, \ubeta]$ and homogeneous carpool disutility $\gamma$.\\
\end{enumerate}

We further impose two assumptions on the latency functions for the simplicity of the calculation:
\begin{enumerate}
    \item The latency function for the ordinary lane and the HOT lane are the same.
    \item Both latency function is linear in $\frac{x}{\rho}$, the average flow on each lane.
\end{enumerate}
That is,
\begin{align*}
    C_o(x; \rho) = C_h(x; \rho) :=  C(\frac{x}{\rho}) \quad \text{ for some linear function } C,
\end{align*}
where
\begin{align*}
    C(\bar{x}) = a\bar{x}+b \quad \text{ for some } a \geq 0, b\geq 0.
\end{align*}

% We start with the case where the latency function is linear and the preference distribution is simple. We say that the preference distribution is simple when both value of time and carpool disutility are homogeneous, or one of the value of time and carpool disutility is homogeneous and the other one is uniformly distributed. Given the traffic flow $x$ of a single lane, there exists non-negative real numbers $a, b$ such that the latency function can be expressed as \[
%     C(x) = ax + b.
% \]
% When the preference distribution is simple, we are able to give a closed form solution for optimal toll price $\tau$ that minimizes average travel time time, minimizes average emission, or maximizes total revenue.

\subsubsection{Homogeneous Value of Time and Homogeneous Carpool Disutility}

If both of the value of time and carpool disutility are homogeneous, then the equilibrium is reached when equation \eqref{eq:homo-equi} is satisfied.
\begin{equation} \label{eq:homo-equi}
    \beta \left( C\left(\frac{D\sigma_o^*}{1 - \rho}\right) - C\left(\frac{D(\sigma_{toll}^* + \frac{1}{A}\sigma_{pool}^*)}{\rho}\right) \right) = \min(\tau, \gamma).
\end{equation}

When the toll price $\tau$ is smaller than the carpool disutility $\gamma$, agents split between taking the ordinary lane and paying the toll to use HOT, while nobody carpools. While $\tau \leq \gamma$, increasing toll price will discourage more people from paying the toll and they will move to the ordinary lane. We remark that under the assumption that the latency is a function of vehicle flows {\em per lane}, minimum average travel time and minimum average emission can both be achieved when the vehicle flow is the same across all lanes, which is induced by $\tau = 0$. 

On the other hand, when $\tau > \gamma$, all people taking the HOT lane carpool, while nobody pays the toll to use the HOT. Increasing the toll price when $\tau > \gamma$ therefore has no impact on the average travel time, average emission, or total revenue. By comparing the objective values achieved in two regimes ($\tau \leq \gamma$ and $\tau > \gamma$), we obtain proposition \ref{thm:fixed-beta-fixed-gamma}.

\begin{proposition} \label{thm:fixed-beta-fixed-gamma}
    Assume the latency function is linear with parameters $a, b > 0$ and the HOT capacity is $\rho$. If all agents have homogeneous value of time $\beta$ and homogeneous carpool disutility $\gamma$, then optimal toll price $\tau$ that minimizes average travel time or average emission is $\ugamma$, while the optimal $\tau$ that maximizes total revenue is $\min\{\frac{a\beta D}{2(1 - \rho)}, \gamma\}$
\end{proposition}

\subsubsection{Homogeneous Value of Time and Uniform Carpool Disutility}

If the value of time is homogeneous and the carpool disutility is uniformly distributed with $\gamma \sim [\lgamma, \ugamma]$, then the equilibrium is reached when equation \eqref{eq:fixed-beta-unif-gamma-equi} is satisfied.
\begin{equation} \label{eq:fixed-beta-unif-gamma-equi}
    \beta \left( C\left(\frac{D\sigma_o^*}{1 - \rho}\right) - C\left(\frac{D(\sigma_{toll}^* + \frac{1}{A}\sigma_{pool}^*)}{\rho}\right) \right) = \tau.
\end{equation}
For agents whose carpool disutility is smaller than the toll price $\gamma < \tau$, they will all carpool. Otherwise, for agents with $\gamma \geq \tau$, they will either pay the toll price or take the ordinary lane.

The average emission is a convex function with respect to $\tau$, while the total revenue is a concave function with respect to $\tau$. Nevertheless, when the objective is to minimize the average travel time, the monotonicity of the objective function w.r.t the $\tau$ depends on the sensitivity of the latency function w.r.t the flow (i.e. the slope $a$ when the latency function is linear). If the slope is small, the average travel time is a convex function w.r.t $\tau$. If the slope is large enough, then the average travel time decreases monotonically w.r.t $\tau$. Proposition \ref{thm:fixed-beta-unif-gamma} illustrates the optimal toll price for achieving the minimum average travel time, minimum average emission, or maximum total revenue, under different sensitivity of the latency function.

\begin{proposition} \label{thm:fixed-beta-unif-gamma}
Assume the latency function is linear with parameters $a, b > 0$ and the HOT capacity is $\rho$. If all agents have homogeneous value of time $\beta$ and uniformly distributed carpool disutility $\gamma \sim [\lgamma, \ugamma]$ with $\lgamma, \ugamma \geq 0$, then optimal toll price $\tau$ that
    \begin{enumerate}
        \item Minimizes average travel time: \[
            \tau = \begin{cases}
                \min\left\{\frac{(1 - \frac{1}{A})\left[1 - \frac{1}{a D\beta}\lgamma (1 - \rho)\right]}{\frac{2}{a D\beta}(1 - \rho)\left[\frac{1}{a D\beta}\rho(\ugamma - \lgamma) - (1 - \frac{1}{A})\right]}, \ugamma \right\} & \text{If } a < \frac{\rho(\ugamma - \lgamma)}{D \beta (1 - \frac{1}{A})}\\
                \ugamma & \text{If } a \geq \frac{\rho(\ugamma - \lgamma)}{D \beta (1 - \frac{1}{A})}\\
            \end{cases}
        \]
        \item Minimizes average emission: \[
            \tau = \min\left\{\frac{\frac{1 - \frac{1}{A}}{\ugamma - \lgamma} \left[2a D \frac{\ugamma - \frac{1}{A}\lgamma}{\ugamma - \lgamma} + b\right]}{2\left[\frac{a D}{(\ugamma - \lgamma)^2}(1 - \frac{1}{A})^2 + \frac{\rho(1 - \rho)}{a D\beta^2} \right]}, \ugamma \right\}.
        \]
        \item Maximizes total revenue: \[
            \tau = \min\left\{\frac{\ugamma - (\ugamma - \frac{1}{A}\lgamma)(1 - \rho)}{2\left[1 + \frac{1}{a D\beta}\rho(1 - \rho)(\ugamma - \lgamma) - (1 - \frac{1}{A})(1 - \rho) \right]}, \ugamma \right\}.
        \]
    \end{enumerate}
\end{proposition}

\ruifan{how to discuss this?}

\subsubsection{Uniform Value of Time and Homogeneous Carpool Disutility} \hfill

When agents have homogeneous carpool disutility and uniform distribution for value of time, there are two different equilibrium regime depends on the value of toll price $\tau$: If $\tau < \gamma$, no one will carpool and agents will split between $R_{o}$ and $R_{toll}$; If $\tau > \gamma$, no one will pay the toll and agents will split between $R_{o}$ and $R_{pool}$.

If $\tau < \gamma$,  no agent will carpool. An agent with preference $(\beta, \gamma)$ will take the ordinary lane if $\beta C_{\delta}(\sigma^*) < \tau$, and will pay the toll if $\beta C_{\delta}(\sigma^*) > \tau$. Since $\beta$ is uniformly distributed in $[\lbeta, \ubeta]$, the fraction of people taking the ordinary lane is $(\tau/C_\delta(\sigma^*) - \lbeta)/(\ubeta-\lbeta)$. Therefore, $\sigma^* = (\sigma^*_{toll}, \sigma^*_{pool}, \sigma^*_{o})$ is solved by 
\begin{align*}
    \begin{cases}
        & \sigma^*_{pool} = 0\\
        &\sigma^*_o = \frac{\tau/C_\delta(\sigma^*) - \lbeta}{\ubeta-\lbeta}\\
        &\sigma^*_o+\sigma^*_{toll} = 1
    \end{cases}.
\end{align*}

If $\tau > \gamma$, no agent will pay the toll. An agent with preference $(\beta, \gamma)$ will take the ordinary lane if $\beta C_{\delta}(\sigma^*) < \gamma$, and will carpool if $\beta C_{\delta}(\sigma^*) > \gamma$. Since $\beta$ is uniformly distributed in $[\lbeta, \ubeta]$, the fraction of people taking the ordinary lane is $(\gamma/C_\delta(\sigma^*) - \lbeta)/(\ubeta-\lbeta)$. Therefore, $\sigma^* = (\sigma^*_{toll}, \sigma^*_{pool}, \sigma^*_{o})$ is solved by 
\begin{align*}
    \begin{cases}
        & \sigma^*_{pool} = 0\\
        &\sigma^*_o = \frac{\gamma/C_\delta(\sigma^*) - \lbeta}{\ubeta-\lbeta}\\
        &\sigma^*_o+\sigma^*_{toll} = 1
    \end{cases}.
\end{align*}

We can then write the equilibrium outcome $\sigma^*$ and the three objectives $\Ltravel, \Lemission, R$ in terms of $\tau$, and compute the optimal $\tau$ for the three objectives, respectively.

\begin{proposition} \label{thm:fixed-gamma}
    If all agents have uniform value of time $\beta \sim [\lbeta, \ubeta]$ and homogeneous carpool disutility $\gamma$. The optimal $\tau$ for the three different objective can be summarized as follows.
    \begin{enumerate}
        \item total travel time $\Ltravel(\tau, \rho)$: $\Ltravel(\tau, \rho)$ is increasing with $\tau$ for $\tau < \gamma$, is discontinuous at $\tau = \gamma$, and does not change for $\tau > \gamma$.
        \begin{align*}
            \tau^* = \begin{cases}
             0  &\text{if } \Ltravel(0, \rho)< \Ltravel(\gamma, \rho)\\
             \tau \text{ for any } \tau> \gamma & \text{otherwise}
            \end{cases},
        \end{align*}
        where $\Ltravel(\gamma, \rho)$ is the total travel time when all agents split between paying the toll or taking the ordinary lane.
        \item total emission $\Lemission(\tau, \rho)$: $\Lemission(\tau, \rho)$ is increasing with $\tau$ for $\tau < \gamma$, is discontinuous at $\tau = \gamma$, and does not change for $\tau > \gamma$.
        \begin{align*}
            \tau^*  =\begin{cases}
             0  &\text{if } \Lemission(0, \rho)<\Lemission(\gamma, \rho)\\
             \tau \text{ for any } \tau> \gamma & \text{otherwise}
            \end{cases},
        \end{align*}
        where $\Ltravel(\gamma, \rho)$ is the total travel time when all agents split between paying the toll or taking the ordinary lane.
        \item maximizing total revenue $R(\tau, \rho)$: $R(\tau, \rho)$ is concave with $\tau$ for $\tau < \gamma$, is discontinuous at $\tau = \gamma$, is $0$ for $\tau > \gamma$.
        \[\tau^* = \min\{\tau_R, \gamma\}\]
        % \[\tau^* =\begin{cases}
        %     \tau_R \quad &\text{ if } \tau_R < \gamma\\
        %     \gamma &\text{ otherwise}
        % \end{cases} ,\]
        where
        \begin{align*}
     \tau_R&=aD\frac{1}{(\ubeta-\lbeta)\rho(1-\rho) }\left(-\frac{1}{9}(( \rho^2-4\rho+1 )(\ubeta-\lbeta)^2-(2\rho-1)(\ubeta-\lbeta)+1)+\sqrt{\Delta_R}\right)
\end{align*}
and $\Delta_R = \frac{4}{81}(( \rho^2-4\rho+1 )(\ubeta-\lbeta)^2-(2\rho-1)(\ubeta-\lbeta)+1)^2+\frac{4}{9}(1 - (1-\rho)(\ubeta-\lbeta))^2 (1+ (\ubeta-\lbeta))\rho (\ubeta-\lbeta) $.\\
(At $\tau = \gamma$, agents taking the HOT lane are indifferent between paying the toll and carpooling, we assume that they will all choose to pay the toll.)
    \end{enumerate}
\end{proposition}

In summary, optimal toll price $\tau$ for minimizing total travel time is achieved either at $\tau = 0$, in which case all agents split between paying the toll price or the ordinary lanes, or at any $\tau > \gamma$, in which case all agents split between carpooling and the ordinary lanes. Therefore, we only need to compare two values $L(0,\rho)$ and $L(\gamma, \rho)$ to find the optimal toll price $\tau$. The total revenue is concave with respect to the toll price $\tau$, and is $0$ for $\tau > \gamma$. If the revenue first increase and then decrease with $\tau$, then the optimal toll price $\tau$ achieved at the maximum point of the concave function; if the revenue is increasing with $\tau$ for all $\tau < \gamma$, then the optimal toll price $\tau$ is $\tau = \gamma$.

% \subsection{General Latency Functions and Preference Distributions} \label{sec:design-general}
% Under general latency functions and preference distributions, it is impossible to give a closed form solution to the optimal toll price that achieves minimum average travel time, minimum average emission, or maximum total revenue, because these objective functions are all non-convex or non-concave w.r.t the toll price $\tau$. Nevertheless, it can still be solved numerically using mathematical programs with equilibrium constraints \cite{luo_pang_ralph_1996}.

% In order to make the computation tractable, we discretize value of times into $m$ chunks $\beta_1, \dots, \beta_m$, and discretize carpool disutilities into $n$ chunks $\gamma_1, \dots, \gamma_n$. Let the density of each grid of $(\beta_i, \gamma_j)$ be $f_{ij}$, where $\sum_{i = 1}^m \sum_{j = 1}^n f_{ij} = 1$. For each combination of $(\beta_i, \gamma_j)$, define its strategy set as $\sigma_{ij} \in \mathbb{R}^3_+$ such that $\sigma_{ij1} + \sigma_{ij2} + \sigma_{ij3} = 1$, where these 3 $\sigma_{ij}$ correspond to the fraction of people with value of time $\beta_i$ and carpool disutility $\gamma_j$ taking the ordinary lane, paying the toll, and carpooling resp. 

% Define $A_o, A_{toll}, A_{pool} \in \mathbb{R}^{m \times n \times 3}$ as adjacency matrices that label the entries corresponding to population that take ordinary lane, pay the toll, and carpool resp. Define $F_o, F_{toll}, F_{pool} \in \mathbb{R}^{m \times n \times 3}$ as the linear maps that aggregate the population that take ordinary lane, pay the toll, and carpool resp. We have \[
%     F_o[ijk] = \begin{cases}
%         f_{ij} & k = 0\\
%         0 & k = 1, 2\\
%     \end{cases},\ F_{toll}[ijk] = \begin{cases}
%         f_{ij} & k = 1\\
%         0 & k = 0, 2\\
%     \end{cases},\ F_{pool}[ijk] = \begin{cases}
%         f_{ij} & k = 2\\
%         0 & k = 0, 1\\
%     \end{cases}
% \]

% The ordinary latency can therefore be written as \[
%     C_o\left(\sum_{i = 1}^m\sum_{j = 1}^n \sigma_{ij}^1 \right) = C\left(\frac{D}{1 - \rho} \sigma^T F_o \right)
% \] and the HOT latency is defined as \[
%     C_h\left(\sum_{i = 1}^m\sum_{j = 1}^n \left(\sigma_{ij}^2 + \frac{1}{A}\sigma_{ij}^3\right)\right) = C\left(\frac{D}{\rho} \sigma^T (F_{toll} + \frac{1}{A} F_{pool}) \right)
% \]

% Let $P$ be the set of feasible strategies such that \[
%     P = \{x \in \mathbb{R}^{m \times n \times 3}_+ \vert x_{ij1} + x_{ij2} + x_{ij3} = 1, \forall i,j \}.
% \] and define the cost vector $\beta$ such that \[
%     \beta_{ijk}(\tau) = \begin{cases}
%         0 & \text{If }k = 1\\
%         \tau & \text{If }k = 2\\
%         \gamma_j & \text{If }k = 3\\
%     \end{cases}.
% \]

% Given a toll price $\tau$, the equilibrium constraints for a strategy profile $x$ can therefore be formulated as
% \begin{align}
%     & x \in P \label{eq:mpec-feasibility}\\
%     & \forall y \in P,\ C\left(\frac{D}{1 - \rho} F_o^T x \right) F_o \odot (y - x) \nonumber \\
%     +& \left[C\left(\frac{D}{\rho} (F_{toll} + \frac{1}{A} F_{pool})^T x \right) + \beta(\tau) \right] (F_{toll} + F_{pool}) \odot (y - x) \geq 0 \label{eq:mpec-vi}
% \end{align}

% The optimization program for minimizing average travel time is
% \begin{align*}
%     \min_{x, \tau}&\ C\left(\frac{D}{1 - \rho} F_o^T x \right) F_o^T x + C\left(\frac{D}{\rho} (F_{toll} + \frac{1}{A} F_{pool})^T x \right) (F_{toll} + F_{pool})^T x\\
%     \text{s.t.}&\ \eqref{eq:mpec-feasibility}-\eqref{eq:mpec-vi}
% \end{align*}

% The optimization program for minimizing average emission is
% \begin{align*}
%     \min_{x, \tau}&\ C\left(\frac{D}{1 - \rho} F_o^T x \right) F_o^T x + C\left(\frac{D}{\rho} (F_{toll} + \frac{1}{A} F_{pool})^T x \right) (F_{toll} + \frac{1}{A} F_{pool})^T x\\
%     \text{s.t.}&\ \eqref{eq:mpec-feasibility}-\eqref{eq:mpec-vi}
% \end{align*}

% The optimization program for maximizing total revenue is
% \begin{align*}
%     \max_{x, \tau}&\ D \tau F_{toll}^T x\\
%     \text{s.t.}&\ \eqref{eq:mpec-feasibility}-\eqref{eq:mpec-vi}
% \end{align*}

% These optimization problems can all be solved numerically using the KKT method \cite{mpec_secondtoll}.

% Additionally, we characterize how average travel time and average emission change after a small perturbation of the toll price. It is particularly useful when the traffic authority has already set a toll price on a road segment but wants to improve either one of the objectives without changing the current toll scheme too significantly.

% Let $\epsilon$ be the number of people switch from paying the toll to other options. Let $\eta$ be the ratio of number of people increased in the ordinary lane to $\epsilon$. I.e. The number of people taking the ordinary lane is increased by $\eta \epsilon$ (if $\eta \epsilon$ is negative, then it means that people taking the ordinary lane decreases). 
% % Before we proceed, we need the following lemma:
% % \begin{lemma}
% %     $\eta \in [-1, 1]$.
% % \end{lemma}
% % \begin{proof}
% %     Recall from the comparative static section, as toll price increases, the number of people paying the toll decreases, the number of people carpooling increases, while the number of people taking the ordinary lane can move to either directions. Now we are given that people paying the toll decreases by $\epsilon$ and people taking the ordinary lane increases by $\eta \epsilon$. Therefore, people carpooling increases by $(1 - \eta)\epsilon$.\\
% %     If $\eta > 1$, then $(1 - \eta)\epsilon < 0$, which means that carpool population decreases. This is a contradiction. Therefore, we must have $\eta \leq 1$. On the other hand, suppose $\eta < -1$, then 
% % \end{proof}

% Propositions \ref{prop:emission} and \ref{prop:travel-time} demonstrates that starting at an equilibrium profile, if the fraction of people who changed from toll paying to the ordinary lane is not larger than some threshold, then a small increase in the toll price can lead to a decrease in average emission or average travel time.

% \begin{proposition} \label{prop:emission}
%     Starting at the current toll price that induces an equilibrium $\sigma^* = (\sigma^*_o, \sigma^*_{toll}, \sigma^*_{pool})$. A small increase in the toll price can lead to a decrease in average emission if \[
%         \eta < \frac{(1 - \frac{1}{A}) \frac{\partial }{\partial x}|_{x = D\frac{\sigma^*_{toll} + \frac{\sigma^*_{pool}}{A}}{\rho}} (xC(x))}{\frac{\partial }{\partial x}|_{x = D\frac{\sigma^*_o}{1 - \rho}} (xC(x)) - \frac{\partial }{\partial x}|_{x = D\frac{\sigma^*_{toll} + \frac{\sigma^*_{pool}}{A}}{\rho}} (xC(x))}
%     \]
% \end{proposition}

% \begin{proposition} \label{prop:travel-time}
%     Starting at the current toll price that induces an equilibrium $\sigma^* = (\sigma^*_o, \sigma^*_{toll}, \sigma^*_{pool})$. A small increase in the toll price can lead to a decrease in average travel time if \[
%         \eta < \frac{(1 - \frac{1}{A})\frac{1 - \sigma^*_o}{\rho} \frac{\partial}{\partial x}\vert_{x = D\frac{\sigma^*_{toll} + \frac{\sigma^*_{pool}}{A}}{\rho}}(C(x))}{\left\{\left(C(D\frac{\sigma^*_o}{1 - \rho}) - C(D\frac{\sigma^*_{toll} + \frac{\sigma^*_{pool}}{A}}{\rho}) \right) + \left(\frac{\sigma^*_o}{1 - \rho} \frac{\partial}{\partial x}\vert_{x = D\frac{\sigma^*_o}{1 - \rho}}(C(x)) - \frac{1 - \sigma^*_o}{\rho} \frac{\partial}{\partial x}\vert_{x = D\frac{\sigma^*_{toll} + \frac{\sigma^*_{pool}}{A}}{\rho}}(C(x))\right) \right\}}
%     \]
% \end{proposition}





==> extension_theory.tex <==
We denote $\delta_e = \ell_{o, e} - \ell_{h, e}$ as the time cost difference between the ordinary lane and the HOT lane of segment $e \in e$. Note that here $\delta_e$ is a variable, not a function. Given time difference vector $\delta = (\delta_e)_{e \in E}$ and toll price vector $\tau = (\tau_e^m)_{e \in E, m \in M}$, we can compute the strategy of each agent $a= (\actionoccu, (\actionseg{\segnum})_{\segnum \in [i, j]})$ in population $(i, j)$ with preference parameter $(\beta, \gamma)$. We define function $\Phi_e(\delta) : = \ell_{o, e}(x_{o, e}^*(\delta, \tau)) - \ell_{h, e}(x_{h, e}^*(\delta, \tau))$, where $x_{o, e}^*(\delta, \tau)$ (resp. $x_{h, e}^*(\delta, \tau)$) is the flow induced by equilibrium strategy associated with $\delta, \tau$. Clearly, both the domain and image of the function $\Phi_e$ is closed, and the function $\Phi_e(\cdot)$ is continuous in $\delta$. Thus, from Kakutani's fixed point theorem, the fixed point solution $\delta = \Phi(\delta)$ exists. Note that both side are $|E|$-dimensional vectors. Moreover, the fixed point solution $\delta^*$ is the time cost difference in equilibrium. 

\begin{lemma}
    \begin{align*}
    \frac{\partial \Phi_e(\delta)}{\partial \delta_{e'}} < 0, \quad \forall e, e' \in E.
\end{align*}
\end{lemma}
\begin{lemma}
   The fixed point solution of $\Phi(\delta) = \delta$ is unique. Then, equilibrium strategy is unique. 
\end{lemma}

I think Lemma 1 is true. I am not sure about Lemma 2. I couldn't find the exact theorem that stated this. Lemma 2 is true when $\Phi(\cdot)$ is single dimension, so the problem is does this generalize in multi dimensional case? 

\zhanhao{
    For lemma 2 per se, I believe I have a counterexample. Consider a function of two segments: let the function be \[
        \begin{cases}
            \Phi_1(\delta) = 2 - \delta_1 - 2\delta_2\\
            \Phi_2(\delta) = 2 - 2\delta_1 - \delta_2\\
        \end{cases}
    \] Then, any $\delta$ with $\delta_1 + \delta_2 = 1$ satisfies the fixed point equation $\Phi(\delta) = \delta$.

    By \cite{kellogg1976uniqueness}, we need to verify $\triangledown_{\delta} \Phi(\delta)$ does not have an eigenvalue of $1$ before we can conclude the uniqueness. I struggled a lot at the beginning of the summer trying to prove it but haven't found a way yet.

}
In the above example, what is the domain? Is it guaranteed to be a self-mapping? 

% $\Phi(\delta)=(f(\delta),g(\delta))$. Define $p(\delta)=f(\delta)-\delta_1$, $q(\delta)=g(\delta)-\delta_2$.
% If there exist two solution $\delta$, $\delta'$, assume WLOG $\delta_1$ does not equal to $\delta'_1$. Then $p(\delta)=p(\delta')=0$. Therefore exist some $c$ such that $p'_1((1-c)\delta+c\delta')=0$. Here $p'_1$ is $dp/d\delta_1$. by definition $p'_1((1-c)\delta+c\delta')<0$ cannot be zero

==> numerical_single_seg.tex <==
We calibrate our equilibrium analysis using the data collected from the Northbound of Interstate 880 Highway (I-880) (Fig. \ref{fig:map}) between the Whipple Rd and Hesperian Blvd. The distance of this road segment is 7.16 miles. Vehicles with carpool size of $3$ can use the HOT lane for free, vehicles with carpool size of $2$ need to pay half of the toll price, while vehicles with a single person have pay the full toll price to use the HOT lane.

\begin{figure}[htp]
    \centering
    \includegraphics[width=0.3\linewidth]{plots/map_whipple2hesperian.png}
    \caption{Interstate 880 (I-880) Highway from Whipple Rd to Hesperian Blvd (Encircled in Red)}
    \label{fig:map}
\end{figure}

\subsection{Modeling Setup}
We adopt the framework of the Bureau of Public Roads (BPR) function to characterize the average travel cost per driver (free flow travel time plus congestion time) \cite{ccolak2016understanding}. Given the HOV capacity $\rho$ and an outcome $\sigma = (\sigma_{toll}, \sigma_{pool}, \sigma_o)$, the latency function is given by the BPR function as follows:
\begin{align*}
    &C_o(\sigma_o; \rho) = T_f \cdot \left[ 1 + \left( a \cdot \frac{D \cdot \sigma_o}{V \cdot (1 - \rho)}\right)^b\right]\\
    &C_h(\sigma_{toll}, \sigma_{pool}; \rho) = T_f \cdot \left[ 1 + \left(a \cdot \frac{D \cdot (\sigma_{toll} + \frac{1}{2}\sigma_{pool2} + \frac{1}{3}\sigma_{pool3})}{V \cdot \rho}\right)^b\right]
\end{align*}
where $a$ and $b$ are the BPR coefficients, $T_f$ is the free flow travel time, and $V$ is the capacity. We set $b = 4.0$ following \cite{roads1964traffic, national1950highway}. Calibrating road capacity $V$ directly from the data is tricky, as it requires us to keep track of the number of cars can pass through the road segment per minute with free flow travel time \cite{ccolak2016understanding}. Nevertheless, the flows recorded by the stations tend to underestimate the number, as the traffic demand is sparse during the non-congestion time. Instead, we decide to fit a regression model (with coefficients $\alpha_0, \alpha_1$) in the form of \[
    C(D\sigma; \rho) = \alpha_0 + \left(\alpha_1 \cdot \frac{D\sigma}{\rho} \right)^b = \alpha_0 + \left(\alpha_1 \cdot \frac{f}{\rho} \right)^b,
\]
where $f$ is the flow observed on this road segment.

Next, we seek to model the equilibrium of people taking the ordinary lane $R_o$, pay full toll price ($R_{toll}$), pay half toll price with carpool size of $2$ ($R_{pool2}$), and carpool with size of $3$ ($R_{pool3}$), by a straightforward extension of our framework in \eqref{eq: equilibrium condition}. We let the induced outcome (fraction of people taking an action) be $\sigma_o$, $\sigma_{toll}$, $\sigma_{pool2}$, and $\sigma_{pool3}$ respectively. We let the preference parameters for an agent be $(\beta, \gamma_2, \gamma_3)$, where $\beta$ is the value of time, $\gamma_2$ is the carpool disutility for carpooling of size $2$, and $\gamma_3$ is the carpool disutility for adding the third person into the car, given the condition that there are already two people in the car. The cost of agent with preference parameters $(\beta, \gamma_2, \gamma_3)$ for playing action $R_i \in \{R_o, R_{toll}, R_{pool2}, R_{pool3}\}$ is therefore given as 
\begin{align*}
    c_{\gamma}^{\beta}(R_{toll}; \sigma) =& \beta \cdot C_h\left(\left(\sigma_{toll} + \frac{\sigma_{pool2}}{2} + \frac{\sigma_{pool3}}{3} \right) D; \rho\right) + \tau,\\
    c_{\gamma}^{\beta}(R_{pool2}; \sigma) =& \beta \cdot C_h\left(\left(\sigma_{toll} + \frac{\sigma_{pool2}}{2} + \frac{\sigma_{pool3}}{3} \right) D; \rho\right) + \gamma_2 + \frac{\tau}{2},\\
    c_{\gamma}^{\beta}(R_{pool3}; \sigma) =& \beta \cdot C_h\left(\left(\sigma_{toll} + \frac{\sigma_{pool2}}{2} + \frac{\sigma_{pool3}}{3} \right) D; \rho\right) + \gamma_2 + \gamma_3,\\
    c_{\gamma}^{\beta}(R_{o}; \sigma) =& \beta \cdot C_o\left(\sigma_{o} D; 1 - \rho\right).
\end{align*}
\ruifan{should it be $\tau/4$ in $pool_{2}$?}

We assume the preference distribution of agents are piecewise uniform in terms of the value of time $\beta$, the carpool disutility for 2 persons $\gamma_2$, and the carpool disutility of 3 persons $\gamma_3$. The population of agents can be discretized into $I$ cubes, in each cube $i$, the value of time is uniformly distributed within $[\lbeta^i, \ubeta^i]$, the carpool disutility for 2 persons is uniformly distributed within $[\lgamma_2^i, \ugamma_2^i]$, and the carpool disutility for 3 persons is uniformly distributed within $[\lgamma_3^i, \ugamma_3^i]$. We assume each cube $i$ of agents has a density $h_i > 0$, where $\sum_{i = 1}^I h_i = 1$.

At equilibrium, the equations \eqref{eq:numerical-sigma-o}-\eqref{eq:numerical-total-fraction} hold.

\ruifan{Should it be $\sigma_{toll}$ in the RHS of first equation?}

\begin{align}
    \int_{\text{Cube }i}\ \mathbb{I}\left(\beta^i \cdot (C_o^t - C_h^t) > \tau_t,\ \gamma_2^i > 0.75 \tau_t,\ \gamma_2^i + \gamma_3^i > \tau_t \right) d(\beta^i, \gamma_2^i, \gamma_3^i) =& \sigma_o^{i, t}, \  \forall i = 1,\dots,I, \forall t, \label{eq:numerical-sigma-toll}\\
    \int_{\text{Cube }i}\ \mathbb{I}\left(\beta^i \cdot (C_o^t - C_h^t) > 0.25 \tau_t + \gamma_2^i,\ \gamma_2^i < 0.75 \tau_t,\ \gamma_3^i > 0.25 \tau_t \right) d(\beta^i, \gamma_2^i, \gamma_3^i) =& \sigma_{pool2}^{i, t}, \  \forall i = 1,\dots,I, \forall t, \label{eq:numerical-sigma-pool2}\\
    \int_{\text{Cube }i}\ \mathbb{I}\left(\beta_i \cdot (C_o^t - C_h^t) > \gamma_2^i + \gamma_3^i,\ \gamma_3^i < 0.25 \tau_t,\ \gamma_2^i + \gamma_3^i < \tau_t \right) d(\beta^i, \gamma_2^i, \gamma_3^i) =& \sigma_{pool3}^{i, t}, \  \forall i = 1,\dots,I, \forall t, \label{eq:numerical-sigma-pool3}\\
    \sigma_o^{i, t} + \sigma_{toll}^{i, t} + \sigma_{pool2}^{i, t} + \sigma_{pool3}^{i, t} =& 1,\ \forall i = 1,\dots,I, \forall t, \label{eq:numerical-sigma-o}\\
    \sum_{i = 1}^I h_i \cdot \vec{\sigma}^{i, t} =& \vec{\sigma}^t, \forall t \label{eq:numerical-sigma-vec}\\
    D_t\sigma_o^t =& f_o^t, \forall t \label{eq:numerical-flow-o}\\
    D_t\left(\sigma_{toll}^t + \frac{1}{2}\sigma_{pool2}^t + \frac{1}{3}\sigma_{pool3}^t\right) =& f_{HOT}^t, \forall t \label{eq:numerical-flow-hot}\\
    %\frac{1 - \rho}{\rho}\left(\frac{C_o^t - \alpha_0}{C_h^t - \alpha_0}\right)^{\frac{1}{b}}\left(\sigma_{toll}^t + \frac{1}{2}\sigma_{pool2}^t + \frac{1}{3}\sigma_{pool3}^t \right) =& \sigma_o^t \label{eq:numerical-ordinary-over-hov}\\
    \frac{\sum_t D_t \sigma_{pool2}^t}{\sum_t D_t \left(\sigma_{toll}^t + \frac{1}{2}\sigma_{pool2}^t + \frac{1}{3}\sigma_{pool3}^t\right)} =& r_{2} \label{eq:numerical-pool2-over-hot}\\
    \frac{\sum_t D_t \sigma_{pool3}^t}{\sum_t D_t \left(\sigma_{toll}^t + \frac{1}{2}\sigma_{pool2}^t + \frac{1}{3}\sigma_{pool3}^t\right)} =& r_{3} \label{eq:numerical-pool3-over-hot}\\
    \sigma_o^t + \sigma_{toll}^t + \sigma_{pool2}^t + \sigma_{pool3}^t =& 1, \forall t \label{eq:numerical-total-fraction}
\end{align}

$\tau_t$ is the toll price at time $t$. $C_o^t$ and $C_h^t$ are the estimated travel time from Whipple Rd to Hesperian Blvd at time $t$, which is calibrated by the sum of estimated travel times from all segments on this road that are divided by the stations. The estimated travel time between two stations is calibrated by using the station length divided by the average traveling speed measured by the station at time $t$ for the ordinary lanes and the HOT lanes respectively. Within each cube of agents, since we assume the preference parameters are uniformly distributed, the strategy profiles corresponds to the area of parameters where each strategy has the lowest cost \eqref{eq:numerical-sigma-toll}-\eqref{eq:numerical-sigma-o}. $r_{2}$ ($r_{3}$) is the ratio of the fraction of people carpool with size $2$ (size $3$ resp.) over the people using HOT lanes, but we only have its data at the daily level. Therefore, we constrain that the fraction of people taking HOT lanes carpool with size $2$ and size $3$ at the daily level, with the equations \eqref{eq:numerical-pool2-over-hot} and \eqref{eq:numerical-pool3-over-hot}.

We measure the total congestion by the average travel time of all travelers: \[
    T(\tau, \rho) := (\sigma_{toll} + \sigma_{pool2} + \sigma_{pool3}) \cdot C_{h}(\sigma_{toll}, \sigma_{pool2}, \sigma_{pool3}; \rho) + \sigma_o \cdot C_o(\sigma_o; \rho).
\]

Similarly, the average emissions from all travelers is computed as \[
    E(\tau, \rho) := (\sigma_{toll} + \frac{1}{2} \sigma_{pool2} + \frac{1}{3}\sigma_{pool3}) \cdot C_{h}(\sigma_{toll}, \sigma_{pool2}, \sigma_{pool3}; \rho) + \sigma_o \cdot C_o(\sigma_o; \rho).
\] 

Additionally, we can compute the total toll revenue as \[
    R(\tau, \rho) := D \cdot \sigma_{toll} \cdot \tau.
\]

Last but not least, we measure the average utility cost of all travelers as
\begin{align*}
    U(\tau, \rho) :=& \int \left[\sigma_o^i \cdot \left(\beta^i C_o(\sigma_o, \rho) \right) \right. \\
    +& \sigma_{toll}^i \cdot \left(\beta^i C_{h}(\sigma_{toll}, \sigma_{pool2}, \sigma_{pool3}; \rho) + \tau \right)\\
    +& \sigma_{pool2}^i \cdot \left(\beta^i C_{h}(\sigma_{toll}, \sigma_{pool2}, \sigma_{pool3}; \rho) + \gamma_2^i + 0.5\tau \right)\\
    +& \left. \sigma_{pool3}^i \cdot \left(\beta^i C_{h}(\sigma_{toll}, \sigma_{pool2}, \sigma_{pool3}; \rho) + \gamma_2^i + \gamma_3^i \right) \right] d(\beta^i, \gamma_2^i, \gamma_3^i).
\end{align*}

\subsection{Data Calibration}

We have a dataset of the number of cars recorded by each station per 5-minute from the California Department of Transportation \footnote{https://pems.dot.ca.gov/} for each workday from March 2021 to August 2021. To mitigate the noise, we aggregate those 5-minute data into per-hour vehicle volume of each station. Then, we take the average among all stations on the road segment from Whipple Rd to Hesperian Blvd to obtain the per-hour traffic flow $f_o^t$ and $f_{HOT}^t$ of this road segment for the ordinary lanes and the HOT lanes. 

Additionally, we compute the per-lane travel time between each pair of adjacent stations by dividing the station length by the per-lane average speed recorded every 5 minutes. We then sum over the travel times across all such segments that cover the Whipple Rd to Hesperian Blvd to obtain the expected travel time of the entire road segment for every 5 minutes. We take an average of those 5-minute expected travel times within each hour to obtain the average travel time for each hour. Then, we compute the average travel time of ordinary lanes $C_o^t$ and the average travel time of HOT lanes $C_h^t$ by averaging over the average travel time of lanes of corresponding types. 

We feed those data into the regression model and then we obtain $\alpha_1 = 7.076 \times 10^{-4}$ and $\alpha_0 = 0.7906$ mins.

Based on equations \eqref{eq:numerical-flow-o}, \eqref{eq:numerical-flow-hot}, and \eqref{eq:numerical-total-fraction}, we can obtain \eqref{eq:numerical-total-demand}
\begin{equation} \label{eq:numerical-total-demand}
    D_t = \frac{f_o^t + f_{HOT}^t}{\sigma_o^t + \sigma_{toll}^t + \frac{1}{2}\sigma_{pool2}^t + \frac{1}{3}\sigma_{pool3}^t}, \forall t.
\end{equation}

Using the average travel times $C_o^t, C_h^t$ calibrated from the real dataset, we can compute the strategy profile $\vec{\sigma}^{i, t} = (\sigma_o^{i, t}, \sigma_{toll}^{i, t}, \sigma_{pool2}^{i, t}, \sigma_{pool3}^{i, t})$ of agents in each cube $i$ using equations \eqref{eq:numerical-sigma-toll}-\eqref{eq:numerical-sigma-o}. Then, rearranging the equations \eqref{eq:numerical-sigma-vec}-\eqref{eq:numerical-flow-hot}, we can obtain the equation \eqref{eq:numerical-flow-strategy}.
\begin{equation} \label{eq:numerical-flow-strategy}
    f_{HOT}^t \sum_{i = 1}^I h_i \sigma_o^{i, t} = f_o^t \sum_{i = 1}^I h_i \left(\sigma_{toll}^{i, t} + \frac{1}{2} \sigma_{pool2}^{i, t} + \frac{1}{3}\sigma_{pool3}^{i, t} \right), \forall t.
\end{equation}

We use a least square solver to obtain numerical solutions to equations \eqref{eq:numerical-flow-strategy}, \eqref{eq:numerical-pool2-over-hot}, \eqref{eq:numerical-pool3-over-hot}, and then we can obtain the calibrated density $h_i$ for each cube $i$ of agents.

% Verification of Calibration Results
Among all the travelers, $54\%$ of them have low value of time and low carpool disutilities: $\beta \sim Unif[0, 0.5]$, $\gamma_2 \sim Unif[0, 1]$, $\gamma_3 \sim Unif[0, 1]$. Additionally, there are $43\%$ of travelers have high value of time and high carpool disutilities: $25\%$ have $\beta \sim Unif[0.5, 1]$, $\gamma_2 \sim Unif[1, 2]$, $\gamma_3 \sim Unif[0, 1]$, $11\%$ have $\beta \sim Unif[0.5, 1]$, $\gamma_2 \sim Unif[1, 2]$, $\gamma_3 \sim Unif[1, 2]$, and $7\%$ have $\beta \sim Unif[0.5, 1]$, $\gamma_2 \sim Unif[3, 4]$, $\gamma_3 \sim Unif[1, 2]$. Last but not least, there are around $3\%$ of travelers have high value of time and low carpool disutilities: $\beta \sim Unif[0.5, 1]$, $\gamma_2 \sim Unif[0, 1]$, $\gamma_3 \sim Unif[0, 1]$. 

Using the calibrated preference density, we obtain the strategy profiles of all travelers using equations \eqref{eq:numerical-sigma-vec}. Then, we compute the travelers' demand per hour for each workday using equation \eqref{eq:numerical-total-demand}. We plotted the average demand for each hour of a workday from 5 am to 7 pm with the 95\% confidence band in figure \ref{fig:demand}. Starting in the early morning, the demand increases and peaks at 2-3 pm, then it starts to decrease until late afternoon.

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{plots/demand.png}
    \caption{Travelers' demand across workdays}
    \label{fig:demand}
\end{figure}

As a sanity check of our calibration, we compare the strategy profile we obtained from the equilibrium against the actual strategy profile at the daily level. Among all travelers taking the HOT lane, we compare the fraction of them carpooling with a size of $2$ and the fraction of them carpooling with a size of $3$. We plotted the moving average of the equilibrium strategies with a window of $2$ weeks. Figure \ref{fig:strategy} demonstrates that our calibrated strategy profile at equilibrium stays closely with the actual one.

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{plots/strategy.png}
    \caption{Travelers' daily level strategy profile at equilibrium v.s. the actual strategy profile}
    \label{fig:strategy}
\end{figure}

\subsection{Optimal Design of Toll Price and HOT Capacity}

We consider an 1-hour time interval (5-6 pm) during the evening rush hour on workdays. The average travel time is 12 mins if taking the ordinary lanes and 9 mins if taking the HOT lane. The total demand at 5-6 pm is $6672$ agents.

We discretize the feasible region of toll price $\tau$ and the capacity fraction $\rho$. In particular, we choose the set $\rho \in\{ \frac{1}{4}, \frac{2}{4}, \frac{3}{4}\}$ since the highway has four lanes. Additionally, we set the toll price within the range of $0$ and $15$ dollars discretized by $\$0.1$. 

For each pair of $(\tau, \rho)$, we compute the equilibrium strategies, the average driving time $T(\tau, \rho)$, the average emissions $E(\tau, \rho)$, and the total toll revenue $R(\tau, \rho)$. In Figure \ref{fig:toll-effect}, we plot the changes of average travel time per traveler, average emission per traveler, and total revenue collected from tolls at 5-6 pm on a workday with respect to the toll price. As the toll price increase, both average travel time and the average emission first decrease and then increase, for all 3 possible HOT lane capacities. Nevertheless, the total revenue is a concave function with respect to the toll price for all 3 possible HOT lane capacities. 

Currently, one out of four lanes on I-880 is the HOT lane, which corresponds to the blue curve ($\rho = 0.25$). The optimal toll price that minimizes the average travel time, average emission, and average utility cost are all $\$8.0$, while the toll price that maximizes the total revenue is $\$1.5$. The optimal average travel time, average emission, total revenue, and average utility cost achieved are $8.86$ mins, $6.85$ mins, $\$1529$, and $\$4.51$ respectively. The toll price currently charged between 5-6 pm on the road segment from Whipple Rd to Hesperian Blvd (North Bound) has an average of $\$4.7$ and is upper bounded by $\$7.0$.

The effect of congestion minimization, emission minimization, and revenue maximization can be enhanced if we increase the HOT lane capacity, as illustrated in Figure \ref{fig:toll-effect}. If the HOT lane capacity increases to $0.5$ (2 out of 4 lanes being HOT), the optimal toll prices that correspond to congestion minimization, emission minimization, utility cost minimization are $\$8.0$, and the optimal toll price that maximizes the revenue is $\$1.5$. The corresponding optimal average travel time, average emission, average utility cost, and total revenue are $7.65$ mins, $5.17$ mins, $\$4.21$, and $\$3073$. If the HOT lane capacity increases to $0.75$ (3 out of 4 lanes being HOT), then the optimal toll prices that correspond to congestion minimization, emission minimization are $\$8.0$, while the optimal toll price that leads to utility cost minimization is $\$3.0$. The optimal toll price that maximizes the total revenue is $\$1.5$. The corresponding optimal average travel time, average emission, average utility cost, and total revenue are $7.23$ mins, $4.14$ mins, $\$4.26$, and $\$4024$.

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.4\linewidth]{plots/3d_latency_vs_toll.png}
    \includegraphics[width=0.4\linewidth]{plots/3d_emission_vs_toll.png}\\
    \includegraphics[width=0.4\linewidth]{plots/3d_utility_vs_toll.png}
    \includegraphics[width=0.4\linewidth]{plots/3d_revenue_vs_toll.png}
    \caption{The change of average travel time, average emission, average utility cost, and total revenue w.r.t toll price}
    \label{fig:toll-effect}
\end{figure}

Setting a very high toll price during the rush hour can effectively mitigate the total travel time and total emission, while the total revenue will be modest as few travelers are incentivized to pay the toll price. However, traffic authority also needs to generate enough revenue from toll collection to support local transportation infrastructures. Therefore, we use the Pareto front to demonstrate the tradeoff between congestion minimization and toll revenue, and the tradeoff between emission minimization and toll revenue.


In Figure \ref{fig:pareto_latency}, we plot the Pareto front of the tuple of $(T, R)$ (marked as the black dashed line), which demonstrates the tradeoff between congestion minimization and toll revenue faced by the authority. The Figure \ref{fig:pareto_emission} shows the Pareto front of the tuple of $(E, R)$ that illustrates the tradeoff between emission minimization and toll revenue. Figure \ref{fig:pareto_utility} illustrates how traveler's average utility cost tradeoff with revenue maximization. Additionally, we plot the Pareto front of $(T, R)$, $(E, R)$, and $(U, R)$ for each feasible capacity allocation $\rho$. We can see that as we increase the number of HOV lanes, we effectively increase the toll revenue while decreasing the total congestion, emission, and utility cost. However, fixing the HOV lane capacity, congestion, emission, or utility cost minimization can also lead to a decrease in total revenue.

\begin{figure}[htb]
    \centering
    \begin{subfigure}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{plots/pareto_latency_combo.png}
        \caption{$T(\tau, \rho)$ v.s. $R(\tau, \rho)$.}
        \label{fig:pareto_latency}
    \end{subfigure}
    \begin{subfigure}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{plots/pareto_emission_combo.png}
        \caption{$E(\tau, \rho)$ v.s. $R(\tau, \rho)$.}
        \label{fig:pareto_emission}
    \end{subfigure}
    \begin{subfigure}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{plots/pareto_utility_combo.png}
        \caption{$U(\tau, \rho)$ v.s. $R(\tau, \rho)$.}
        \label{fig:pareto_utility}
    \end{subfigure}
    \caption{Pareto fronts of congestion minimization, emission minimization, utility cost minimization, and revenue maximization}
    \label{fig:pareto_fronts}
\end{figure}

\subsection{Time-Variant Optimal Pricing Scheme}

The traffic demand varies by a lot at different times of a day. We apply the same model to each hour from 5 am to 7 pm of a workday. One challenge with the time-variant HOT design is that the equilibrium profile of the current batch of vehicles can affect the congestion level of the new imminently arrived vehicles. Therefore, if we design the pricing scheme of HOT on a very small time scale, the pricing decision at the current time will be impacted by the pricing decisions in previous time steps. We remark that most trips can be finished within half an hour. Therefore, by considering the equilibrium in per hour time scale, we can mitigate the impact from previous pricing decisions.

For each hour, we compute the optimal toll prices that induce the minimum congestion, minimum average emission, and maximum total revenue. We fix the HOT capacity as $0.25$ to match the current HOT capacity on I-880 and we compare our optimal toll prices with the actual toll prices given by the traffic authority (figure \ref{fig:toll-dynamic}).

\begin{figure}[ht!]
    \centering
    \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=0.4\linewidth]{plots/min_congestion.png}
        \includegraphics[width=0.4\linewidth]{plots/dynamic_congestion_improvement.png}
        \caption{Congestion minimization.}
        \label{fig:dynamic-congestion}
    \end{subfigure}\\
    %
    \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=0.4\linewidth]{plots/min_emission.png}
        \includegraphics[width=0.4\linewidth]{plots/dynamic_emission_improvement.png}
        \caption{Emission minimization.}
        \label{fig:dynamic-emission}
    \end{subfigure}\\
    %
    \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=0.4\linewidth]{plots/min_utility_cost.png}
        \includegraphics[width=0.4\linewidth]{plots/dynamic_utility_cost_improvement.png}
        \caption{Utility cost minimization.}
        \label{fig:dynamic-utility-cost}
    \end{subfigure}\\
    %
    \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=0.4\linewidth]{plots/max_revenue.png}
        \includegraphics[width=0.4\linewidth]{plots/dynamic_revenue_improvement.png}
        \caption{Revenue maximization.}
        \label{fig:dynamic-revenue}
    \end{subfigure}
    \caption{Optimal toll price for minimum congestion, minimum emission, minimum utility cost, and maximum revenue for each hour of a work day.}
    \label{fig:toll-dynamic}
\end{figure}

In figure \ref{fig:toll-dynamic}, the plots on the left column shows the optimal toll prices for congestion minimization, emission minimization, utility cost minimization, and revenue maximization for each hour from 5 am to 7 pm of a workday. The red curves are the optimal toll prices, whereas the blue dots are the average toll prices implemented in the real world, along with its 95\% confidence regions. The plots on the right column quantifies the improvement in these four objectives by adjusting the toll price from the current average toll prices to the optimal toll prices. The blue bars denote the percentage of improvements in the objectives, while the red curves denote the improvements in actual dollars or minutes of all travelers.

We find that the overall trend of optimal pricing for congestion, emission, and utility cost minimization matches to the actual prices \ref{fig:dynamic-congestion}-\ref{fig:dynamic-utility-cost}. In order to minimize the congestion, emission, and utility cost, the toll prices in the afternoon should be higher than the toll prices in the morning. The optimal toll prices are uniformly higher than the actual toll prices at all times except for 5 am, where a $\$0$ toll price is optimal. By adjusting the actual toll prices to the optimal toll prices, we can obtain up to 18\% improvement in congestion, 27\% improvement in emission, and 16\% improvement in utility cost. Adding up the objective improvements of all travelers, adjusting the toll price can save up to 10k minutes of travel time, 14k minutes of emission time, and $\$4$k of utility costs. Nevertheless, all these large improvements occur during the morning hours. The positive effect of toll price adjustment in congestion, emission, and utility cost is modest during the afternoon hours. The reason is that the actual toll prices during the afternoon are already very high, so most of the travelers taking the HOT lane are already carpooling. Therefore, further increasing the toll price cannot incentivize a significant number of travelers to switch their strategies from toll-paying to carpooling.

On the other hand, the optimal toll price for revenue maximization should be more stable and stay within $\$1$-$\$2$ throughout the day \ref{fig:dynamic-revenue}. The optimal toll price is very close to the actual toll prices during the morning hours. However, by decreasing the actual toll prices in the afternoon, we can achieve up to $800\%$ increase in the revenue, which amounts of up to $\$1750$ of increase in total revenue collected per hour.

==> objective_optimization.tex <==
\subsection{Minimizing Total Emission}
\begin{definition}
    The total emission $L: \mathbb{R}_+^2 \rightarrow \mathbb{R}_+$ is defined as 
    \begin{equation} \label{eq:total-emission}
        L(\tau, \rho) := D \cdot \sigma^*_o C_o(\sigma^*_o \cdot D; 1 - \rho) + D \cdot (\sigma^*_{toll} + \frac{\sigma^*_{pool}}{A}) C_o((\sigma^*_{toll} + \frac{\sigma^*_{pool}}{A}) \cdot D; \rho),
    \end{equation}
    where $(\sigma^*_{toll}, \sigma^*_{pool}, \sigma^*_o)$ is the equilibrium strategy given toll price $\tau$ and HOV capacity $\rho$.
\end{definition}
To find the optimal design of HOT that minimizes the total emission, we need to solve the following optimization problem:
\begin{align*}
    \min_{\tau, \rho}&\ L(\tau, \rho)\\
    \text{s.t.}\ & \eqref{eq:b-fixed_point-toll}-\eqref{eq:b-fixed_point-o}\\
    & \tau \geq 0
\end{align*}
Nevertheless, solving this optimization problem directly is hard, as for each combination of $\tau$ and $\rho$, we have to solve for the system of equations \eqref{eq:b-fixed_point-toll}-\eqref{eq:b-fixed_point-o}. Luckily, under some mild assumptions, we are able to convert this into a much simpler optimization problem that does not require solving the system of equations \eqref{eq:b-fixed_point-toll}-\eqref{eq:b-fixed_point-o}, as demonstrated in theorem \ref{thm:emission-dual}.

\begin{theorem} \label{thm:emission-dual}
    Assume the latency function is given in the form \[
        C_o(x; \rho) = C_h(x; \rho) := C(\frac{x}{\rho}),
    \] where $C: \mathbb{R}_+ \rightarrow \mathbb{R}_+$ is a non-decreasing convex function.\\
    For a fixed HOV capacity $\rho$, finding the toll price $\tau$ that minimizes the total emission \eqref{eq:total-emission} is equivalent to finding the toll price $\tau$ that maximizes the fraction of agents using HOV:
    \begin{equation}
        \max_{\tau}\ \sigma^*_{toll} + \sigma^*_{pool}.
    \end{equation}
\end{theorem}
\zhanhao{
    Alternatively, instead of assuming $C_o(x; \rho) = C_h(x; \rho) := C(\frac{x}{\rho})$, we can assume
    \begin{enumerate}
        \item $C_o(x; \rho) = C_h(x; \rho)$
        \item For any $\rho, x_1, x_2$ with $C(x_1, 1 - \rho) \geq C(x_2, \rho)$, we have \[
            \frac{\partial}{\partial x} |_{x = x_1} (x C(x, 1 - \rho)) \geq \frac{\partial}{\partial x} |_{x = x_2} (x C(x, \rho))
        \]
    \end{enumerate}
}

\subsection{Maximizing Revenue}
\begin{definition}
    The revenue function $R: \mathbb{R}_+^2 \rightarrow \mathbb{R}_+$ is defined as
    \begin{equation} \label{eq:revenue}
        R(\tau, \rho) := \tau D \cdot \sigma^*_{toll},
    \end{equation}
    where $(\sigma^*_{toll}, \sigma^*_{pool}, \sigma^*_o)$ is the equilibrium strategy given toll price $\tau$ and HOV capacity $\rho$.
\end{definition}

\subsection{Pareto Front}
To find a toll price $\tau$ that jointly optimizes the total emission and revenue while holding the HOV capacity $\rho$ fixed, we can work with the objective function 
\begin{equation} \label{eq:joint}
    \max_{\tau}\ \sigma^*_{toll} + \sigma^*_{pool} + \lambda \tau \sigma^*_{toll},
\end{equation}
where $\lambda \geq 0$ is a hyperparameter allowing the transportation system planner to assign a weights between total emission minimization and revenue maximization.



\subsection{Proof of Theorem \eqref{thm:emission-dual}}
\noindent \emph{Proof:}
The main idea is to demonstrate that starting from an arbitrary {\em equilibrium} strategy profile $(\sigma^*_{toll}, \sigma^*_{pool}, \sigma^*_o)$, any other equilibrium profiles with higher $\sigma^*_o$ will have a higher total emission. Therefore, in order to find the optimal HOV design that has the minimum total emission, it is equivalent to find the equilibrium strategy profile with lowest $\sigma^*_o$. With a fixed HOV lane capacity $\rho$, the only way to move from an equilibrium to another is to increase or decrease the toll price $\tau$. We first consider the case where we increase the toll price $\tau$.

As we increase the toll price $\tau$ to $\tau'$ while holding the HOV lane capacity $\rho$ fixed, the total emission \eqref{eq:total-emission} and fraction of people using ordinary lane $\sigma^*_o$ at equilibrium will either both increase or both decrease.

We have already argued in section \ref{sec:comparative_statics} that as toll price $\tau$ increase, $\sigma^*_{toll}$ decreases and $\sigma^*_{pool}$ increases, while $\sigma^*_o$ may change in either direction. We will discuss the scenarios where $\sigma^*_o$ increases and where $\sigma^*_o$ decreases separately. We overload the expression for total emission by \[
    L(\sigma^*_{toll}, \sigma^*_{pool}, \sigma^*_o) := L(\tau, \rho),
\] where $(\sigma^*_{toll}, \sigma^*_{pool}, \sigma^*_o)$ is the equilibrium profile rendered by $\tau$ and $\rho$.

\medskip

\noindent \emph{If $\sigma^*_o$ decreases}:\\
Assume that after the toll price $\tau$ increases to $\tau'$, the new equilibrium becomes $(\sigma'^*_{toll}, \sigma'^*_{pool}, \sigma'^*_o)$. In section \ref{sec:proof-comparative}, we have shown that as toll price $\tau$ increases, the congestion level at HOV lanes will certainly decrease, i.e. \[
    C_h((\sigma'^*_{toll} + \frac{\sigma'^*_{pool}}{A})D; \rho) < C_h((\sigma^*_{toll} + \frac{\sigma^*_{pool}}{A})D; \rho).
\]



Hence, we can prove that the total emission will decrease if $\sigma^*_o$ decreases:
\begin{align*}
    L(\sigma^*_{toll}, \sigma^*_{pool}, \sigma^*_o) =& \sigma'^*_o D \cdot C_o(\sigma'^*_o D; 1 - \rho) + (\sigma'^*_{toll} + \frac{\sigma'^*_{pool}}{A})D \cdot C_h((\sigma'^*_{toll} + \frac{\sigma'^*_{pool}}{A})D; \rho)\\
    <& \sigma^*_o D \cdot C_o(\sigma^*_o D; 1 - \rho) + (\sigma'^*_{toll} + \frac{\sigma'^*_{pool}}{A})D \cdot C_h((\sigma'^*_{toll} + \frac{\sigma'^*_{pool}}{A})D; \rho)\\
    <& \sigma^*_o D \cdot C_o(\sigma^*_o D; 1 - \rho) + (\sigma^*_{toll} + \frac{\sigma^*_{pool}}{A})D \cdot C_h((\sigma^*_{toll} + \frac{\sigma^*_{pool}}{A})D; \rho)\\
    =& L(\sigma'^*_{toll}, \sigma'^*_{pool}, \sigma'^*_o)
\end{align*}
Hence, we have shown that when $\sigma^*_{toll}$ decreases and $\sigma^*_{pool}$ increases, the decrease in $\sigma^*_o$ leads to a decrease in total emission. As a result, for any two equilibrium profiles $(\sigma^1_{toll}, \sigma^1_{pool}, \sigma^1_o)$ and $(\sigma^2_{toll}, \sigma^2_{pool}, \sigma^2_o)$ with $\sigma^1_{toll} > \sigma^2_{toll}$, $\sigma^1_{pool} < \sigma^2_{pool}$, and $\sigma^1_o > \sigma^2_o$, we then have $L(\sigma^1_{toll}, \sigma^1_{pool}, \sigma^1_o) > L(\sigma^2_{toll}, \sigma^2_{pool}, \sigma^2_o)$.

\medskip
\noindent \emph{If $\sigma^*_o$ increases}:\\
We abuse the notation by defining \[
	C^{\rho}(x) := C(x \cdot D, \rho)
\] and \[
	C'^{\rho}(x) := \frac{d}{dx} C(x \cdot D, \rho)
\]
Assume that after the toll price increases from $\tau$ to $\tau'$, the equilibrium $\sigma^*_{toll}$ decreases by $\epsilon > 0$, $\sigma^*_o$ increases by $\gamma \epsilon$ and $\sigma^*_{pool}$ increases by $(1 - \gamma)\epsilon$, for some $\gamma \in [0, 1]$. The new emission function can therefore be expressed as
\begin{align*}
    L(\sigma'^*_{toll}, \sigma'^*_{pool}, \sigma'^*_o) =& (\sigma^*_o + \gamma\epsilon) D \cdot C_o((\sigma^*_o + \gamma\epsilon) D; 1 - \rho)\\
    +& (\sigma^*_{toll} + \frac{\sigma^*_{pool}}{A} - [(1 - \frac{1}{A} + \gamma)]\epsilon)D \cdot C_h((\sigma^*_{toll} + \frac{\sigma^*_{pool}}{A} - [(1 - \frac{1}{A} + \gamma)]\epsilon)D; \rho)
\end{align*}
Since the latency function $C$ is convex and its input $x$ is non-negative, it is easy to show that \[
    \frac{\partial^2}{\partial x^2} (xC^{\rho}(x)) \geq 0.
\]
As a result, for any $0 < x_1 < x_2$, we have
\begin{equation} \label{eq:proof-thm3-derivative-increase}
    \frac{\partial }{\partial x}|_{x = x_1} (xC(x)) = C(x_1) + x_1 C'(x_1) \leq C(x_2) + x_2 C'(x_2) = \frac{\partial }{\partial x}|_{x = x_2}.
\end{equation}

We will show that the total emission $L(\tau')$ will increase as we increase $\sigma'^*_o$, i.e. increasing $\gamma$, by analyzing the first-order derivative:
\begin{align*}
    \frac{\partial}{\partial \gamma} L(\sigma^*_{toll}, \sigma^*_{pool}, \sigma^*_o) =& \epsilon C^{1 - \rho}(\sigma^*_o + \gamma \epsilon) + \epsilon (\sigma^*_o + \gamma \epsilon) C'^{1 - \rho}(\sigma^*_o + \gamma \epsilon)\\
    -& \epsilon C^{\rho}(\sigma^*_{toll} + \frac{\sigma^*_{pool}}{A} - [(1 - \frac{1}{A}) + \gamma]\epsilon)\\
    -& \epsilon (\sigma^*_{toll} + \frac{\sigma^*_{pool}}{A} - [(1 - \frac{1}{A}) + \gamma]\epsilon) C'^{\rho}(\sigma^*_{toll} + \frac{\sigma^*_{pool}}{A} - [(1 - \frac{1}{A}) + \gamma]\epsilon)\\
    =& \epsilon \left\{\frac{\partial }{\partial x}|_{x = \frac{\sigma^*_o + \gamma\epsilon}{1 - \rho}} (xC(x)) - \frac{\partial }{\partial x}|_{x = \frac{\sigma^*_{toll} + \frac{\sigma^*_{pool}}{A} - [(1 - \frac{1}{A}) + \gamma]\epsilon}{\rho}} (xC(x)) \right\}\\
    \overset{(1)}{\geq}& \epsilon \left\{\frac{\partial }{\partial x}|_{x = \frac{\sigma^*_o}{1 - \rho}} (xC(x)) - \frac{\partial }{\partial x}|_{x = \frac{\sigma^*_{toll} + \frac{\sigma^*_{pool}}{A}}{\rho}} (xC(x)) \right\}\\
    \overset{(2)}{\geq}& 0
\end{align*}
The inequality (1) is because \[
    \frac{\sigma^*_o + \gamma\epsilon}{1 - \rho} \geq \frac{\sigma^*_o}{1 - \rho}
\] and \[
    \frac{\sigma^*_{toll} + \frac{\sigma^*_{pool}}{A} - [(1 - \frac{1}{A}) + \gamma]\epsilon}{\rho} < \frac{\sigma^*_{toll} + \frac{\sigma^*_{pool}}{A}}{\rho}
\]. The inequality (2) is because for any equilibrium profile, the latency at HOV lane must be no larger than the latency at ordinary lane, so we have \[
    C^{1 - \rho}(\sigma^*_o) \geq C^{\rho}(\sigma^*_{toll} + \frac{\sigma^*_{pool}}{A}).
\]
By the assumption in theorem \eqref{thm:emission-dual} that the latency function $C^{\rho}(x)$ takes the form of $C(\frac{x}{\rho})$ for a non-decreasing function, it is then equivalent to \[
    \frac{\sigma^*_o}{1 - \rho} \geq \frac{\sigma^*_{toll} + \frac{\sigma^*_{pool}}{A}}{\rho}.
\]
Inequalities (1) and (2) then follow immediately after applying \eqref{eq:proof-thm3-derivative-increase}.\\
Hence, we have shown that when $\sigma^*_{toll}$ decreases and $\sigma^*_{pool}$ increases, an increase in $\sigma^*_o$ leads to a non-decreasing trend in total emission. As a result, for any two equilibrium profiles $(\sigma^1_{toll}, \sigma^1_{pool}, \sigma^1_o)$ and $(\sigma^2_{toll}, \sigma^2_{pool}, \sigma^2_o)$ with $\sigma^1_{toll} > \sigma^2_{toll}$, $\sigma^1_{pool} < \sigma^2_{pool}$, and $\sigma^1_o < \sigma^2_o$, we then have $L(\sigma^1_{toll}, \sigma^1_{pool}, \sigma^1_o) \leq L(\sigma^2_{toll}, \sigma^2_{pool}, \sigma^2_o)$.

In the case where the toll price decreases, we have $\sigma^*_{toll}$ increases and $\sigma^*_{pool}$ decreases, and the arguments to $\sigma^*_o$ can be made symmetric to the case where the toll price increases. As a result, for any two equilibrium profiles $(\sigma^1_{toll}, \sigma^1_{pool}, \sigma^1_o)$ and $(\sigma^2_{toll}, \sigma^2_{pool}, \sigma^2_o)$ with $\sigma^1_{toll} < \sigma^2_{toll}$, $\sigma^1_{pool} > \sigma^2_{pool}$, and $\sigma^1_o < \sigma^2_o$, we then have $L(\sigma^1_{toll}, \sigma^1_{pool}, \sigma^1_o) < L(\sigma^2_{toll}, \sigma^2_{pool}, \sigma^2_o)$. On the other hand, for any two equilibrium profiles $(\sigma^1_{toll}, \sigma^1_{pool}, \sigma^1_o)$ and $(\sigma^2_{toll}, \sigma^2_{pool}, \sigma^2_o)$ with $\sigma^1_{toll} < \sigma^2_{toll}$, $\sigma^1_{pool} > \sigma^2_{pool}$, and $\sigma^1_o > \sigma^2_o$, we then have $L(\sigma^1_{toll}, \sigma^1_{pool}, \sigma^1_o) \geq L(\sigma^2_{toll}, \sigma^2_{pool}, \sigma^2_o)$.
 
To sum up, starting at an arbitrary equilibrium profile, it can be changed to another equilibrium profile by either increasing or decreasing the toll price, and we have argued that in all possible direction of changes, i.e.
\begin{enumerate}
    \item Toll price increases:
    \begin{enumerate}
        \item $\sigma^*_{toll}$ decreases, $\sigma^*_{pool}$ increases, $\sigma^*_o$ decreases.
        \item $\sigma^*_{toll}$ decreases, $\sigma^*_{pool}$ increases, $\sigma^*_o$ increases.
    \end{enumerate}
    \item Toll price decreases:
    \begin{enumerate}
        \item $\sigma^*_{toll}$ increases, $\sigma^*_{pool}$ decreases, $\sigma^*_o$ increases.
        \item $\sigma^*_{toll}$ increases, $\sigma^*_{pool}$ decreases, $\sigma^*_o$ decreases.
    \end{enumerate}
\end{enumerate}
an increase in $\sigma^*_o$ will lead to a non-decreasing trend in total emission. Therefore, minimizing the total emission is equivalent to minimizing the fraction of people taking the ordinary lane at equilibrium, which is equivalent to maximizing the fraction of people taking the HOV lane at equilibrium, i.e. \[
    \max_{\tau} \sigma^*_{toll} + \sigma^*_{pool}.
\]

\hfill $\square$

